Hierarchical Imitation and Reinforcement Learning

We study how to effectively leverage expert feedback to learn sequential decision-making policies. We focus on problems with sparse rewards and long time horizons, which typically pose significant challenges in reinforcement learning. We propose an algorithmic framework, called hierarchical guidance, that leverages the hierarchical structure of the underlying problem to integrate different modes of expert interaction. Our framework can incorporate different combinations of imitation learning (IL) and reinforcement learning (RL) at different levels, leading to dramatic reductions in both expert effort and cost of exploration. Using long-horizon benchmarks, including Montezuma's Revenge, we demonstrate that our approach can learn significantly faster than hierarchical RL, and be significantly more label-efficient than standard IL. We also theoretically analyze labeling cost for certain instantiations of our framework.

==> app_notation.tex <==

\begin{table}[t]\caption{Table of Notation}
	\vskip -0.1in
	\begin{small}
		\begin{center}% used the environment to augment the vertical space
			% between the caption and the table
			\begin{tabular}{r c p{5cm} }
				\toprule
				$g$ & $\triangleq$ & subgoal, $g\in \Gcal$\\% = \{ 1,\ldots,G\}$\\
				$\mu(s), \muopt(s)$ & $\triangleq$ & learner and expert meta-controller, mapping states to goals\\ %; \quad $g\leftarrow \mu(s)$\\
				$\pi_g(s), \pigopt(s)$ & $\triangleq$ & learner and expert policy for subgoal $g$, mapping states to primitive actions\\
				%$\pi^*_g$ & $\triangleq$ & expert policy for subgoal $g$\\
				%$\mu^*$ & $\triangleq$ & expert meta-controller\\
				%$\omega$ & $\triangleq$ & termination condition, $\omega\in [0,1]$\\
				$\beta_g(s)$, $\beta_g^\star(s)$ & $\triangleq$ & learner and expert termination function for subgoal $g$, mapping states to $\True/\False$\\
				%$[a,\omega]$ & $\triangleq$ & action and termination for policy $\pi_g$\\
				%& &$[a,\tau] \leftarrow \pi_g(s)$ \\
				%$s^\prime$ & $\triangleq$ & decision point states\\
				$H_\fu$, $H_\lo$, $H_\hi$ & $\triangleq$ & full, $\lo$-level, and $\hi$-level horizons\\
				$\tau$ & $\triangleq$ & $\lo$-level trajectory, which contains primitive actions  and $|\tau| \le H_\lo$\\%experience tuples for each subgoal segment $\tau = \{ (s, [a, \omega])\}$\\
				$\tau_\hi$ & $\triangleq$ &  $\hi$-level trajectory, which contains subgoals and $|\tau| \le H_\hi$ \\
				$\tau_\fu$ &  $\triangleq$ &  full trajectory, which contains primitive actions and $|\tau_\fu| \le H_\fu$ \\
				$\sigma$ &  $\triangleq$ &  hierarchical trajectory, which contains subgoals in addition to $\tau_\fu$\\
				$\Dhi$ & $\triangleq$ & meta-controller data (aggregated)\\
				$\Dg$ & $\triangleq$ & subgoal $g$ data (aggregated)\\
				\bottomrule
			\end{tabular}
		\end{center}
	\end{small}
	\label{tab:notation_table}
	\vskip -0.2in
\end{table}

%When we only receive demonstration data at the high level, and must utilize reinforcement learning at the low level, then our setting can be viewed as an instance of learning under weak demonstration feedback.
%Some alternative ways to elicit weaker feedback include preference-based or gradient-based learning \citep{furnkranz2012preference,loftin2016learning,christiano2017deep}. Also somewhat related to weak expert supervision is the approach of~\citet{andreas2016modular}, which addresses the multi-task reinforcement learning problem by assuming access to symbolic descriptions of subgoals, without knowing what those symbols mean or how to execute them.
%More generally, it would be interesting to explore other forms of weak demonstration feedback in structured policy classes.



%\begin{table}[t]\caption{Full Table of Notation}
%	\begin{center}% used the environment to augment the vertical space
%		% between the caption and the table
%		\begin{tabular}{r c p{5cm} }
%			\toprule
%			$g$ & $\triangleq$ & subgoal, $g\in \Gcal = \{ 1,\ldots,G\}$\\
%			$\mu(s), \muopt(s)$ & $\triangleq$ & learner and expert meta-controller at state $s$\\ %; \quad $g\leftarrow \mu(s)$\\
%			$\pi_g(s), \pigopt(s)$ & $\triangleq$ & learner and expert policy for subgoal $g$ at state $s$\\
%			%$\pi^*_g$ & $\triangleq$ & expert policy for subgoal $g$\\
%			%$\mu^*$ & $\triangleq$ & expert meta-controller\\
%			%$\omega$ & $\triangleq$ & termination condition, $\omega\in [0,1]$\\
%			$\beta_g(s)$, $\beta_g^\star(s)$ & $\triangleq$ & learner and expert termination function for subgoal $g$ at state $s$\\
%			%$[a,\omega]$ & $\triangleq$ & action and termination for policy $\pi_g$\\
%			%& &$[a,\tau] \leftarrow \pi_g(s)$ \\
%			%$s^\prime$ & $\triangleq$ & decision point states\\
%			$H_\fu$, $H_\lo$, $H_\hi$ & $\triangleq$ & full, $\lo$-level, and $\hi$-level horizons\\
%			 $\tau=(s_1,a_1,\dotsc,s_H,a_H,s_{H+1})$ & $\triangleq$ & $\lo$-level trajectory, which contains primitive actions  and $|\tau| \le H_\lo$\\
%			$\tau_\hi$ & $\triangleq$ &  $\hi$-level trajectory, which contains subgoals and $|\tau| \le H_\hi$ \\
%			$\tau_\fu$ &  $\triangleq$ &  full trajectory, which contains primitive actions and $|\tau_\fu| \le H_\fu$ \\
%			$\sigma$ &  $\triangleq$ &  hierarchical trajectory, which contains subgoals in addition to $\tau_\fu$\\
%			$\Dhi$ & $\triangleq$ & meta-controller data (aggregated)\\
%			$\Dg$ & $\triangleq$ & subgoal $g$ data (aggregated)\\
%			\bottomrule
%		\end{tabular}
%	\end{center}
%	\label{tab:notation_table_long}
%\end{table}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "icml_paper.tex"
%%% End: 
